Unsupervised Object Detection with LiDAR Clues

Despite the importance of unsupervised object detection, to the best of our knowledge, there is no previous work addressing this problem. One main issue, widely known to the community, is that object boundaries derived only from 2D image appearance are ambiguous and unreliable. To address this, we exploit LiDAR clues to aid unsupervised object detection. By exploiting the 3D scene structure, the issue of localization can be considerably mitigated. We further identify another major issue, seldom noticed by the community, that the long-tailed and open-ended (sub-)category distribution should be accommodated. In this paper, we present the first practical method for unsupervised object detection with the aid of LiDAR clues. In our approach, candidate object segments based on 3D point clouds are firstly generated. Then, an iterative segment labeling process is conducted to assign segment labels and to train a segment labeling network, which is based on features from both 2D images and 3D point clouds. The labeling process is carefully designed so as to mitigate the issue of long-tailed and open-ended distribution. The final segment labels are set as pseudo annotations for object detection network training. Extensive experiments on the large-scale Waymo Open dataset suggest that the derived unsupervised object detection method achieves reasonable accuracy compared with that of strong supervision within the LiDAR visible range. Code shall be released.

==> algos/ground.tex <==
\begin{algorithm}[H]
\DontPrintSemicolon
\SetAlgoLined
\SetAlgoNoEnd
\LinesNumbered
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwFunction{bfs}{BFS}
\SetKwFunction{Proj}{ProjectPointCloud}

\newcommand{\var}{\texttt}

\Input{Elevation map $E\in\mathbb{R}^{(R-1)\times C}$}
\Input{Maximum elevation angle difference $\epsilon$}
\Output{Ground map $G\in\{0,1\}^{R\times C}$}


initialize $G \leftarrow \mathbf{0}^{R\times C}$\;
\For {$c \leftarrow 1$ \KwTo $C$} {
	\If(){$E_{1,c} < 45^{\circ}$ and $G_{1, c} \ne 1$ }{
		\bfs{G, E, $1$, c}
	}
}


\SetKwProg{Fn}{function}{:}{}
\Fn{\bfs{G, E, r, c}}{
	\var{queue.push($\{r, c\}$)}\;
	\While{\textup{$\var{queue}$} is not empty}{
		$\{r, c\} \leftarrow \var{queue.pop()}$\;
		
		$G_{r,c} \leftarrow 1$\;
		
		\For{$\{r_n, c_n\} \in$ \textup{4-neighbor($\{r, c\}$)}}{
			\If{$|E_{r,c} - E_{r_n,c_n}| < \epsilon$}{
				\textup{\var{queue.push($\{r_n,c_n\}$)}}
			}
		}
	}
}

\caption{Ground Removal}
\label{algo:ground}
\end{algorithm}


==> algos/instance.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\SetAlgoNoEnd
\LinesNumbered
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwFunction{bfs}{BFS}

\newcommand{\var}{\texttt}

\Input{Range image $D\in\mathbb{R}^{R\times C}$}
\Input{Maximum steepness angle $\theta$}
\Output{Label map $L\in\mathbb{Z}_+^{R\times C}$}

initialize $L\leftarrow \mathbf{0}^{R\times C}$ \;
initialize $\var{label} \leftarrow 1$ \;

\For{$r=1\leftarrow R$}{
	\For{$c=1\leftarrow C$}{
		\If{$L_{r,c}=0$}{
			\bfs{D, L, r, c, \textup{\var{label}}}\;
			\var{label} $\leftarrow$ \var{label} $+1$
		}
	}
}

\SetKwProg{Fn}{function}{:}{}
\Fn{\bfs{D, L, r, c, \textup{\var{label}}}}{
	\var{queue.push($\{r, c\}$)}\;
	$L_{r,c}\leftarrow \var{label}$\;
	\While{\textup{$\var{queue}$} is not empty}{
		$\{r, c\} \leftarrow \var{queue.pop()}$\;		
		\For{$\{r_n, c_n\} \in$ \textup{4-neighbor($\{r, c\}$)}}{
			$d_1\leftarrow\max(D_{r,c}, D_{r_n,c_n})$\;
			$d_2\leftarrow\min(D_{r,c}, D_{r_n,c_n})$\;
			\If{$\beta < \theta$}{
				\textup{\var{queue.push($\{r_n,c_n\}$)}}
			}
		}
	}
}

\caption{Point Cloud Clustering}
\label{algo:instance}
\end{algorithm}


==> algos/propagation.tex <==
{\SetArgSty{textnormal}
\begin{algorithm*}
\SetAlgoLined
\SetAlgoNoEnd
\SetNoFillComment
\LinesNumbered
\SetKwInOut{Input}{input}
\SetKwInOut{Parameter}{parameters }
\SetKwInOut{Output}{output}
\SetKwFunction{IoF}{IoF}
\SetKwFunction{Proj}{ProjectPointCloud}
\SetKwFunction{Queue}{Queue}
\SetKwFunction{Enqueue}{Enqueue}
\SetKwFunction{Dequeue}{Dequeue}
\SetKwFunction{Empty}{Empty}
\SetKwFunction{Avg}{Average}
\SetKwFunction{Bbox}{BoundingBox}
\SetKwFunction{IoU}{IoU}
\SetKwComment{Comment}{$\triangleright$\ }{}

\Input{candidate segments $\{S_t\}_{t=1}^{T}$ and corresponding labels $\{Y_t\}_{t=1}^{T}$, where $S_t = \{\varsigma_t(j)\}_{j=1}^{n_t}$ and $Y_t = \{y_t(j)\}_{j=1}^{n_t}$}
\Input{overall motion fields $\{M_{t\to t+1}^\text{scene}\}_{t=1}^{T-1}$ and $\{M_{t\to t-1}^\text{scene}\}_{t=2}^{T}$}
\Parameter{overlap threshold $\eta_\text{match} = 0.8$ for matching segments}
\Output{labels after propagation $\{Y_t\}_{t=1}^{T}$}

\BlankLine
\tcc{Project 3D coordinates to 2D image according to Eq.\ref{eq:projection}.}
\For {each candidate segment $\varsigma_t(j)$} {
    $\zeta'_t(j)$ = \Proj{$\varsigma_t(j)$}\;
}

\BlankLine
\tcc{Initialize a queue with all movable segments.}
$Q =$ \Queue{}\; %\Comment*[r]{Initialize an empty queue.}
\For {each movable segment with $y_t(j) == 1$} {
    Q.\Enqueue{$(t, j)$} \Comment*[r]{\footnotesize enqueue the $j^{th}$ segment at time $t$}
}

\BlankLine
\tcc{Propagate each movable segment forward and backward.}
\While{not Q.\Empty{}}{
    $(t, j)$ = Q.\Dequeue{} \Comment*[r]{\footnotesize dequeue a movable segment}
    \BlankLine
    \tcc{propagation from t to t+1}
    \If {$t < T$} {
        $M_{t\to t+1}^\text{seg}(j)$ = \Avg{$M_{t\to t+1}^\text{scene}(\zeta'_t(j))$} \Comment*[r]{\footnotesize average motion}
        $\zeta'_{t\to t+1}(j)$ = $\zeta'_{t}(j) + M_{t\to t+1}^\text{seg}(j)$ \Comment*[r]{\footnotesize translate segment}
        \For {each unclear segment in time $t+1$ with $y_{t+1}(j') == 0$} {
            $B_{t\to t+1}(j)$ = \Bbox{$\zeta'_{t\to t+1}(j)$}\;
            $B_{t+1}(j')$ = \Bbox{$\zeta'_{t+1}(j')$}\;
            \If {\IoU{$B_{t\to t+1}(j)$, $B_{t+1}(j')$} $>$ $\eta_\text{match}$} {
                $y_{t+1}(j') = 1$ \Comment*[r]{\footnotesize re-labeled as movable}
                Q.\Enqueue{$(t+1, j')$}\;
            }
        }    
    } 
    \BlankLine
    \tcc{propagation from t to t-1}
    \If {$t > 1$} {
        $M_{t\to t-1}^\text{seg}(j)$ = \Avg{$M_{t\to t-1}^\text{scene}(\zeta'_t(j))$} \Comment*[r]{\footnotesize average motion}
        $\zeta'_{t\to t-1}(j)$ = $\zeta'_{t}(j) + M_{t\to t-1}^\text{seg}(j)$ \Comment*[r]{\footnotesize translate segment}
        \For {each unclear segment in time $t-1$ with $y_{t-1}(j') == 0$} {
            $B_{t\to t-1}(j)$ = \Bbox{$\zeta'_{t\to t-1}(j)$}\;
            $B_{t-1}(j')$ = \Bbox{$\zeta'_{t-1}(j')$}\;
            \If {\IoU{$B_{t\to t-1}(j)$, $B_{t-1}(j')$} $>$ $\eta_\text{match}$} {
                $y_{t-1}(j') = 1$ \Comment*[r]{\footnotesize re-labeled as movable}
                Q.\Enqueue{$(t-1, j')$}\;
            }
        }    
    } 
}
\BlankLine
\Return{$\{Y_t\}_{t=1}^{T}$}

\caption{movable Segment Propagation}
\label{algo:propagation}
\end{algorithm*}}


==> algos/rematch.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\SetAlgoNoEnd
\LinesNumbered
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwFunction{IoF}{IoF}
\SetKwFunction{Proj}{ProjectPointCloud}

\Input{A set of camera-projected point cloud segmentations $\{O_i\}$ and corresponding 3D point sets $\{P_i\}$}
\Input{A set of propagated detections $\{D_i^\text{prop}\}$}
\Output{A set of refined detections $\{D_i^+\}$}

$D^+ = \{\}$\;
\For {$D_i \in \{D_i^\text{prop}\}$} {
	$p = \{\}$\;
	\For {$O_i$ in $\{O_i\}$}{
		\If(){\IoF{$O_i$, $D_i$}$>\eta$}{
			$p = p \cup P_i$
		}
	}
	$D^+ = D^+ \cup$ \Proj{p}
}

\caption{Rematch Propagated Detections with Camera-projected Point Cloud Segmentations}
\label{algo:rematch}
\end{algorithm}

